Recursive Deep Prior Video: a Super Resolution algorithm for Time-Lapse Microscopy of organ-on-chip experiments

Biological experiments based on organ-on-chips (OOCs) exploit light Time-Lapse Microscopy (TLM) for a direct observation of cell movement that is an observable signature of underlying biological processes. A high spatial resolution is essential to capture cell dynamics and interactions from recorded experiments by TLM. Unfortunately, due to physical and cost limitations, acquiring high resolution videos is not always possible. To overcome the problem, we present here a new deep learning-based algorithm that extends the well known Deep Image Prior (DIP) to TLM Video Super Resolution (SR) without requiring any training. The proposed Recursive Deep Prior Video (RDPV) method introduces some novelties. The weights of the DIP network architecture are initialized for each of the frames according to a new recursive updating rule combined with an efficient early stopping criterion. Moreover, the DIP loss function is penalized by two different Total Variation (TV) based terms. The method has been validated on synthetic, i.e., artificially generated, as well as real videos from OOC experiments related to tumor-immune interaction. Achieved results are compared with several state-of-the-art trained deep learning SR algorithms showing outstanding performances.

==> img_tikz/fig10.tex <==
\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/UDPV-TV2.png}};
	\spy on (-0.2,0.4) in node [name=c] at (9.3,-4);
	\draw[red,ultra thick,rounded corners] (0.62,0.65) rectangle (0.78,0.75);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV-TVi}};
		
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/UDPV-TV1.png}};
	\spy on (-0.2,0.4) in node [name=c] at (6.2,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV-TVa}};
		
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/UDPV.png}};
	\spy on (-0.2,0.4) in node [name=c] at (3.1,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/DPV.png}};
	\spy on (-0.2,0.4) in node [name=c] at (0,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{DPV}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/RCAN.png}};
	\spy on (-0.2,0.4) in node [name=c] at (9.3,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RCAN}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/ESRGAN.png}};
	\spy on (-0.2,0.4) in node [name=c] at (6.2,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{ESRGAN}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/LR.png}};
	\spy on (-0.2,0.4) in node [name=c] at (3.1,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{LR}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286Sobel/GT.png}};
	\spy on (-0.2,0.4) in node [name=c] at (0,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{GT}};
	
	\end{tikzpicture}
	\caption{\textbf{Real Frame of Videos Type2, x4, Sobel images.} Three regions of interest are also highlighted as blue, green and red squares.}
	
\end{figure}

==> img_tikz/fig9.tex <==
\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/UDPV-TV2.png}};
	\spy on (-0.2,0.4) in node [name=c] at (9.3,-4);
	\draw[red,ultra thick,rounded corners] (0.62,0.65) rectangle (0.78,0.75);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV-TVi}};
		
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/UDPV-TV1.png}};
	\spy on (-0.2,0.4) in node [name=c] at (6.2,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV-TVa}};
		
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/UDPV.png}};
	\spy on (-0.2,0.4) in node [name=c] at (3.1,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RDPV}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/DPV.png}};
	\spy on (-0.2,0.4) in node [name=c] at (0,-4);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{DPV}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/RCAN.png}};
	\spy on (-0.2,0.4) in node [name=c] at (9.3,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{RCAN}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/ESRGAN.png}};
	\spy on (-0.2,0.4) in node [name=c] at (6.2,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{ESRGAN}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/LR.png}};
	\spy on (-0.2,0.4) in node [name=c] at (3.1,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{LR}};
	
	\begin{scope}[spy using outlines={rectangle,red,magnification=2,size=3cm}]
	\node {	\includegraphics[height=3cm]{img_reali/frame286/GT.png}};
	\spy on (-0.2,0.4) in node [name=c] at (0,0);
	\draw[blue] (-0.5,-0.33) rectangle (0.01,0.01);
	\end{scope}
	\node[below of=c, align=center, node distance=2cm] {\textbf{GT}};
	
	\end{tikzpicture}
	\caption{\textbf{Real Frame of Videos Type2, x4}.Three regions of interest are also highlighted as blue, green and red squares.}
	
\end{figure}

==> related_new.tex <==
\section{On image Super Resolution algorithms} \label{related works}

In the field of SR, the Single Image Super Resolution (SISR) task, which is the problem of reconstructing an HR image from a single LR image, has mostly caught the attention among the researchers. In the discrete setting, the single image SR observation model can be fixed as it follows: 

\begin{equation}\label{eq:SISR_problem}
    S x + \eta = y 
\end{equation}

where $S \in \mathbb{R}^{NM \times L^{2}NM}$ is the degradation matrix which links the HR image $x \in \mathbb{R}^{L^{2}MN \times 1}$ to the LR image $y \in \mathbb{R}^{MN \times 1}$, both reshaped as vectors.
%The positive integer $L$, also known as magnification factor, is the square root of ratio between the dimensions of the HR and LR images. 
Moreover, $\eta \in \mathbb{R}^{MN \times 1}$ is the Additive White Gaussian Noise (AWGN) component of standard deviation $\sigma$, which corrupts the LR measurement. Mathematically, the single SR problem is known to be a strongly ill-posed problem \citep{yue2016}. The linear system in \eqref{eq:SISR_problem} is an underdetermined system, thus many HR images are related to the acquired LR image $y$, hence inverting the process described by \eqref{eq:SISR_problem} hasn't a unique solution. Moreover the discrete operator $S$ is known to be badly conditioned, therefore the solution results to be sensible to the presence of noise in the measurement $y$. In the literature, many approaches have been proposed in order to get one of the possible solutions of the single image SR problem. Among them, the interpolation-based methods reallocate the LR image pixels on a finer grid, then the missing pixel values are estimated using interpolation techniques such as Bicubic interpolation and Lanczos resampling \citep{duchon1979}. Even if the interpolation-based methods are computationally cheap, they suffer from accuracy issues since they are not capable to retrieve the missing high frequency details. 
Another common approach in the literature is to add some prior information on the desired HR solution $x$, in order to shrink the space of the possible solutions. This is done in different ways by the algorithms belonging to the class of reconstruction-based SISR and learning-based SISR methods which are currently the state-of-the-art for SISR. 
The class of reconstruction-based methods rewrites the problem \eqref{eq:SISR_problem} as the following unconstrained minimization problem: 
\begin{equation} \label{eq:rec_based}
    x^{*}=\arg \min_{x} \lVert y - Sx \rVert_{2}^{2} + \lambda \rho(x).
\end{equation}
The objective function in \eqref{eq:rec_based} encodes both the information on the fixed observation model  (type of noise, blur, downsampling, etc.) and the prior information on the solution (smoothess, sparsity, etc.) by the first and the second term in the sum, respectively. The scalar parameter $\lambda$ is an hyperparameter which represents a trade-off between the two terms (see \citep{yue2016} and references therein). 
Despite their good performances, their flexibility and their strong mathematical underpinnings, the quality of the reconstruction computed by those methods degrades rapidly when the magnification factor increases.
Learning-based SISR methods utilize Deep Convolutional Neural Network (DCNN) architectures to learn the statistical correlation between the LR and the HR image from an external database of training examples. They attempt to solve the following minimization problem: 
\begin{equation}\label{eq:DL}
    \theta^{*} = \arg \min_{\theta} \mathcal{L}(f_{\theta}(Y), X) 
\end{equation}
where $f_{\theta}$ is a fixed Deep Neural Network architecture with weights $\theta$, $\mathcal{L}$ is a  loss function and  $\lbrace Y,X \rbrace$ is a set of LR and HR  example pairs.  Then, for a given LR image $\Tilde{x}$ \textcolor{red}{perche'non X?} the HR reconstruction $\Tilde{y}$ is obtained as $\Tilde{y}=f_{\theta^{*}}(\Tilde{x})$. 
Deep learning performances are strictly related to the  capacity of the DCNN to extract high-level features and to approximate high-dimensional and complex maps that link the LR image to its well-looking HR counterpart. Moreover, their success is also due to the capacity of these models to handle a big amount of data. Indeed, by means of a sufficiently large training set, these strategies are capable to capture image statistics and to reproduce them. Hereafter, we review some well known and more powerful deep learning methods for SISR belonging to the state-of-the-art. The Enhanced Deep Super-Resolution (EDSR) neural network \citep{EDSR} exploits residual blocks and a pre-trained strategy for different scale factors. The deep Residual Channel Attention Networks (RCAN) \citep{RCAN} introduces residual in residual \textcolor{red}{ripetizione} structures and a channel attention mechanism to adaptively rescale channel-wise features. The Enhanced Super-Resolution Generative Adversarial Networks (ESRGAN) \citep{ESRGAN} is based on adversarial training and is able to reconstruct realistic textures by using perceptual loss. The Progressive Super-Resolution (ProSR) \cite{proSR} method applies multi-scale progressiveness for SISR. It is able to handle higher up-scaling factor with respect to the other state-of-the-art methods by implementing an asymmetric pyramidal structure with more layers. However, there have been introduced proSRs which is a faster version of proSR, and proSRGAN which makes use of adversarial training. 
All the previous methods follow a supervised learning approach, i.e., a set of LR-HR image pairs as examples are needed for the training. In order to obtain good quality HR reconstructions, most of the previous SISR methods usually require a varied set of examples and consequently an overstated computational effort. Moreover, in most cases the trained deep architecture are specialized for a fixed magnification factor, hence the training must be repeated on a different data set if a different magnification factor is needed. 
We also point out  that is quite difficult in real applications either to acquire images of the same scene with different resolutions or dispose of  a varied data set. In addition, they can exhibit instability issues due to the presence of noise in the LR data \citep{wang2020}. SR techniques have also been  developed to reconstruct high-quality videos. Given $N$ consecutive LR frames $(I_{1}, \dots I_{t-1},I_{t},I_{t+1} \dots I_{N})$ of a video clip, the task is to reconstruct an HR version of one of the LR frames taken into account \textcolor{red}{?}. All the real-world Video Super-Resolution (VSR) approaches usually try to make use of spatial and temporal dependencies among video frames, such as motions and color changes. As a consequence, video super-resolution methods aim to align and establish accurate correspondences among multiple frames. The existing methods  model all these dependencies following different approaches (see \citep{wang2020} and references therein). For example in \citep{kappeler2016}, the motion between frames is modelled and estimated by means of learning-based techniques. The implemented architecture exploits additional information due to the subpixel motions among frames, which is possible because a very high-temporal frequency of acquisition is used, i.e. from 15 to 60 frames per second \citep{Nah_2019}. \textcolor{red} {In this work,instead, we focused on TLM videos which are constructed by acquiring frames at fixed time step, from seconds, e.g. 20 s \citep{Comes2019}, to minutes, e.g. every 2 min \citep{nguyen2018dissecting}.}
For this reason, we refer to SISR algorithms as competing methods neglecting the last mentioned video super resolution approaches. Differently from all the aformentioned learning approaches we propose an unsupervised method for TML video Super Resolution avoiding the problem of constructing a dataset. The proposed method combines the reconstructed and the learning based approaches exploiting the a priori information brought by CNN architecture and total variation penalization. Furthermore, a parameter sharing technique is implemented to transfer the knowledge between consecutive frames improving the performances. 
\textcolor{red}{rivedere ultima parte}


